Particle-Laden Fluid on Flow Maps

We propose a novel framework for simulating ink as a particle-laden flow using particle flow maps. Our method addresses the limitations of existing flow-map techniques, which struggle with dissipative forces like viscosity and drag, thereby extending the application scope from solving the Euler equations to solving the Navier-Stokes equations with accurate viscosity and laden-particle treatment. Our key contribution lies in a coupling mechanism for two particle systems, coupling physical sediment particles and virtual flow-map particles on a background grid by solving a Poisson system. We implemented a novel path integral formula to incorporate viscosity and drag forces into the particle flow map process. Our approach enables state-of-the-art simulation of various particle-laden flow phenomena, exemplified by the bulging and breakup of suspension drop tails, torus formation, torus disintegration, and the coalescence of sedimenting drops. In particular, our method delivered high-fidelity ink diffusion simulations by accurately capturing vortex bulbs, viscous tails, fractal branching, and hierarchical structures.

==> backup/rebuttal2_bkup.tex <==
We thank the reviewers for their insightful feedback and constructive suggestions. 

### MOTIVATION
Although our paper does not feature high-resolution simulations or state-of-the-art details set by industrial standards using hybrid methods such as PIC/FLIP, we contend that our research forges a novel path for the graphics community in simulating free-surface flows especially for pure Lagrangian methods. We provided a mathematically rigorous model and a numerically practical solution to solve the free-surface flow problem from the covector (impulse) perspective, which, to our knowledge, has been infeasible in both graphics and physics communities due to the difficulties of directly enforcing accurate boundary conditions on a dynamic free surface. Because of this methodological deficiency, the applications of the covector model have been confined to simulating smoke, which, in our opinion, represents a regrettable gap only because of the emerging difficulties in correctly handling boundary conditions in a new fluid model. We argue that accurately enforcing boundary conditions is an essential first step toward visually appealing simulations and is always acknowledged as a valuable contribution within SIGGRAPH. We demonstrate this with two examples: correctly setting solid boundaries for vortex methods [Yin 2023] and defining free-surface boundaries in Clebsch methods [Xiong 2022].

We make two main contributions: (1) extending covector models to support free-surface flow simulation and (2) developing flow-map methods to facilitate Lagrangian fluid simulation. We achieved these two goals by addressing the mathematical foundation (Equation 8) and providing a numerical solution (Equation 14 and Algorithm 1). Our idea of converting a spacetime boundary integral problem, which requires identifying and integrating quantities on an evolving interface, to a volumetric path integral problem, which can be naturally realized on moving particles, is general to be extended in accommodating other Lagrangian approaches such as SPH. We believe these methodologies are worth sharing with the graphics community.

### RESOLUTION 

Our approach did not achieve high-resolution simulation primarily due to the bottleneck associated with constructing Voronoi diagrams in parallel. The most effective open-source codebase available to us is XXX, which is implemented sequentially on the CPU. Consequently, we did not achieve a resolution improvement comparable to PPM, as we faced the same implementation bottleneck (we noticed the potential solution, XXX, available in the literature, but unfortunately, their codebase is not open-sourced). Although choosing Voronoi diagrams over alternatives, such as SPH particles, may seem an unconventional choice at first glance, it proved to be the only viable option for us at present, according to our experiments. This is because a flow-map solver requires an accurate projection step to obtain a divergence-free velocity field (rather than obtaining an incompressible volume, as implemented in many incompressible SPH solvers) due to its need to integrate pressure along the particle path. 

%We have tested various particle discretizations, such as incompressible SPH, but currently, the only practical technical pathway that meets the standard for accurate projection is using the Voronoi projection step.   

% Zhiqi: I wang to add this to emphasize this issue can be solved
%However, this limitation can be addressed, as there are methods in the literature of high performance to generate Voronoi cell parallelly by GPU[1].(Unfortunately, their code is not open source now.)

%[1] [add the title of that paper here]
%% I do want to say this but I feel it is a bit aggressive. 
%Many new methods, such as PIC/FLIP and PPM, did not surpass the state-of-the-art in terms of their visual results (resolution and/or visual quality) when they were first introduced. However, these approaches provided refreshing perspectives that have benefited the community. 

### EXPOSITION

- Notation

We employ a covector viewpoint instead of "impulse + flow map" to present a geometrically intuitive and mathematically concise derivation from Equation 3 to 6. While it is possible to derive Equation 6 from an impulse perspective, this would require the path integral of Lagrangian pressure with some nontrivial gauge transform. We will be happy to revise Sections 3 and 4 to make them more accessible to the general graphics audience (e.g., by mentioning both perspectives when introducing Equation 6). Equations after Equation 6 were all presented in vector form.

- Timing Statistics

We will include detailed timing statistics in the revision. We have identified that the main bottleneck of our program lies in the generation of the Voronoi diagram, but the time cost incurred by this process is not optimal (as explained previously). We plan to record the time spent on the generation of the Voronoi diagram separately from the time spent on other components. This is to demonstrate the potential efficiency of our method after implementing an efficient Voronoi diagram generation algorithm.

[Bo: I don't think it is necessary to describe these details.]

[Zhiqi: add some brief description of timing here]
[Zhiqi: How about this?]
\textit{
We are pleased to include detailed timing statistics in the revision.  Here we can present some approximate data.  Our simulation sovler can achieve the performance that when running on the V100 GPU, excluding Voronoi generation, each substep, including 400 steps of CG, takes approximately 15 seconds for 480k particles.
}


[Zhiqi: could you put other expositional points here?]  

- Other concerns:  We will address all the other writing and exposition suggestions in our next version, including
    - Fix typos.
    - Fix notation and equation errors.
    - Use vector notation more precisely.
    - Improve color contrast, size and schemes of figures(e.g., Fig 7 covers the caption of Fig 5).
    - Polish the captions of figures.
    - Clarify which model we use(LMCP) and which models are intermediate building blocks(LMLP, SMSP, and LMSP).
    - Use illustrations to articulate the model (e.g., LMSP) more clearly.
    - Clarify reinitialization process and number of boundary layer.
    - Specify the meaning of colors in the image (e.g., Vorticity in Fig 10, velocity in Fig 8 and 9)."

%-   Vortex based method is not suitable for free surface

%Both Reviewer 3 and Reviewer 5 mentioned that adding vortices to fluid with a free surface may not be crucial (with less pronounced visual effects), but studies such as [2] have demonstrated the rich visual effects of vortices in fluids with free surfaces, including sink vortices (as implemented in our cases) and horseshoe vortices. Additionally, although our method and the covector method possess the ability to maintain vortices, our approach is not a vortex-based method, because our computations do not involve vorticity and do not require the conversion from vorticity to velocity.

%[2] A Clebsch Method for Free-Surface Vortical Flow Simulation

%[Bo: we may not need this paragraph, as I already made this point at the beginning. It might not be so meaningful to argue whether important or not to have a free-surface vortex solver]

### COMPARISON WITH OTHER METHODS

- PPM
We compared our approach against PPM in 3 experiments (i.e., Fig 10, 6, 16) to highlight its strengths in preserving vortical structures. We will be happy to incorporate one further comparisons with PPM on free surface examples, including sink vortex example, which refers to the vortex formed at the drain hole when draining a tank of water (see Fig. 12/13). The reason we use this case for comparison is that it is a 3D example with a surface, which allows us to demonstrate the vortex-preserving capability of our method in situations involving free surfaces in three dimensions.

{I think original version is too lengthy}
{We compared our approach against PPM in 3 experiments (i.e., Fig 10, 6, 16) to highlight its strengths in preserving vortical structures. We are happy to further incorporate 3D free surface examples(see Fig. 12/13) comparing with PPM to demonstrate the vortex-preserving capability.}

- Covector
Our comparisons focused on particle-based methods and did not encompass grid-based ones. However, we are open to incorporating additional comparative analyses with the covector method to highlight this disparity. 
{I don't think we can promise comparison with covector.}
{Our comparisons focused on particle-based methods and did not encompass grid-based ones. Considering our method is focuing on extending covector for supporting free surface flow on pure Lagrangian, we think it's hard to perform comparison with grid-based Covector method}

- MPM/FLIP/APIC
We are happy to incorporate one more comparison to PIC/FLIP fluid on free-surface flow simulation: the sink vortex example. The reason for using this example is explained in the "Comparison with PPM" part. 

{We will also compare PIC/FLIP in 2D vortex preservation experiments to highlight the necessity of Covector representation and show a 3D free surface }

### SIMULATION ARTIFACTS

- Floating Wall Particles: These are caused by gaps in particle-based wall boundaries that trap fluid particles. We will address this artifact by applying a small thrust away from the wall.

- Downward Moving Particles in Dam Break: This is a rendering issue, caused by particles not strictly above the ground. We will fix this artifact by adjusting the particle radius and height.

#### INDIVIDUAL COMMENTS

[Zhiqi: TODO]
- R1

    %-   Clarify Which model we use: we use LMCP model and LMLP, SMSP, and LMSP are all intermediate building blocks. 

    -   CFL number: Our CFL condition is consistent with the Power Particle method: CFL = 1. Although our approach is based on Covector Fluid, it is constrained by the implementation of the Power Particle method. As a result, our CFL cannot achieve the same magnitude as Covector (CFL $\ge$ 6). In fact, pure Lagrangian methods, such as SPH, PPM, generally have limited CFL numbers.  For pure Lagrangian methods, high CFL number would lead to rapid particle movement, potentially disrupting the structure of the particle system.

- R2

    %-   Clarify reinitialization process and number of boundary layer: Due to space constraints, our discussion on reinitialization and the boundary layer is relatively concise. Reinitialization involves resetting the starting point of the flow map, as outlined in Algorithm 1, where lines 4 and 5 specify the reinitialization process. The initialization strategy R in line 3 essentially determines "when to perform reinitialization." We use the simplest and most robust reinitialization strategy, which is to perform reinitialization every n substeps (in our experiments, we set n=20).  As for the boundary layer, in our experiments, we set the parameter k to 3. Generally, a larger k  reduces the part computed by the covector fluid method, thereby weakening its ability to maintain vortices.  Therefore, it is advisable to use smaller values of k. In our experiments, we found that k=3 already produces satisfactory results.
    
    %- Color in Fig 10： The red/blue color in fig 10 represent vorticity.  
    
- R3
    
    -   The question of whether there are genuine concerns with the flow map method in the presence of a free surface that need resolution:  In fact, for a Free Surface, the Flow Map faces two challenges. 
    
    The first issue, as mentioned in the introduction section, is the difficulty in tracking the integration of particles at the boundary due to the complex topological changes in the fluid. Reviewer 4 pointed out that in analytical solutions, boundary particles always remain on the boundary. However, in practical simulations, especially when there are drastic deformations at the fluid surface, such as splashing water, this assertion cannot be guaranteed.  Slight error in Covector Method at the free surface can result in significant issues in the simulation, as depicted in Figure 11.

    The second issue with Flow Map is mentioned in Section 7, since the Flow Map method requires the computation of the matrix T, the free-surface boundary lacks sufficient particles to support the calculation of T (lacking an accurate extrapolation for T due to missing particles). 
    
    These two issues collectively contribute to the difficulty in computing free-surface conditions with the Flow Map method. In Figure 11, we conducted an ablation study to demonstrate the necessity of our approach to handling free surfaces in the Flow Map.
    
- R4
    -   Comparison with Sato et al: If space permits, we can add a discussion of Sato et al.'s method. Sato et al.'s method is also a kind of long flow map method, with differences from our approach: (1) Sato et al.'s method is based on the direct integration formula for the Euler equations, while our method is based on the Covector integration formula (Formula 6) for the Euler equations, which better preserves vorticity. (2) The use of the integration formula (Formula 6) better combines the processes of mapping and projection [3] because the pressure term in (6) is integrated as a whole before taking the gradient. This allows for solving the Poisson equation globally for the integrated pressure term to reduce numerical errors accumulated during integration (corresponding to our LMLP). (3) However, LMLP may encounter difficulties in handling boundary conditions. Therefore, we propose Short Mapping, and Proposition 6.1 demonstrates that, for Covector methods, Short Mapping is equivalent to Long Mapping and does not lead to numerical error accumulation. "(4) The Sato et al. method is a grid-based approach, while our method employs a pure Lagrangian method, utilizing the concept that 'particles themselves are the flow map.' Our approach does not require explicit backtracing of the flow map."

    [3] Nabizadeh M S, Wang S, Ramamoorthi R, et al. Covector fluids

    {Do we really need to mention these much detail? I think we can just say Sato is a Eulerian method without using Covector formulation. Hence, it's not suitable for comparison since our focus is solving the problem that covector fluid can't handle free surface simulation.}
    
- R5
    The concerns raised by Reviewer 5 have already been discussed in the shared concerns part.


==> barney_related_works_notes.tex <==
\section{Related works}
\duowen{need to be paraphrased for gauge and flowmap and make particle based fluid shorter.}
\paragraph{Particle-based fluid simulation}

\barney{Connecting neighbors with smoothing kernels carried on particles, Smoothed Particle Hydrodynamics (SPH) emerged as a prevalent technique for simulating fluids in a Lagrangian setting. Since its first introduction to the computer graphics community for the simulation of fire \cite{stam1995depicting}, SPH has been used to simulate various fluid phenomena, including weakly compressible fluids using small time steps \cite{becker2007weakly,ihmsen2011parallel,muller2003particle,solenthaler2008density}. Density-constrained SPH methods adressed the simulation of incompressible flow \cite{ellero2007incompressible,solenthaler2009predictive,macklin2013position,ihmsen2013implicit}.}

\barney{Particle-based methods often suffer from numerical dissipation. Previous work addressed the over-damping of vortices by vorticity confinement, adding a corrective force to the system, artificially reintroducing vorticity \cite{fedkiw2001visual,macklin2013position,lentine2011mass,hong2008bubbles}.}

\barney{Despite all these improvements, particle-based fluid simulation techniques at large remain prone to energy dissipation due to excessive damping, making these ill-suited for scenarios, where the accurate simulation of vortex dynamics is desired.}

\barney{
\cite{de2015power} introduced power particles for the simulation of incompressible fluids. Their geometrically inspired method offers precise pressure solving and an even distribution of particles by describing the fluid motion as a series of well-shaped power diagrams. \cite{zhai2018fluid} accelerated the construction of power diagrams on GPUs and \cite{levy2022partial} applied sphere clamping for handling free-surfaces instead of treat free-surface interactions with ghost particles. Our method builds on the original approach, while greatly improving on vorticity and energy preservation, via utilizing the theory of flow map advection and gauge variable.
}

\barney{
Our method takes inspiration from the power particle method, while greatly improving on energy and vorticity preservation by combining a gauge variable and the theory of flow map advection for simulating fluids.
}

% version after gpt gramma fix
\duowen{Particle-based fluid simulation has drawn attention in graphics community to simulate various fluid beahaviors. Smoothed Particle Hydrodynamics (SPH) \cite{monaghan2005smoothed}, treating particles as material points, was initially employed to simulate weakly compressible fluids using small time steps \cite{stam1995depicting, muller2003particle, becker2007weakly, solenthaler2008density, ihmsen2011parallel}. Subsequently, to model incompressible flows, various density-constrained SPH methods were introduced, utilizing techniques such as Lagrangian multipliers \cite{ellero2007incompressible}, predictive-corrective methods \cite{solenthaler2009predictive}, and iterative solutions using the Position-based Dynamics framework \cite{macklin2013position}. This was further enhanced by \citet{ihmsen2013implicit} through the use of a modified pressure Poisson equation for implicit divergence-free constraint enforcement, later refined by \citet{bender2016divergence} and \citet{band2018pressure} for better density variation and boundary handling. Nonetheless, SPH methods often suffer from excessive damping, leading to energy dissipation, which limits their effectiveness in simulations that focus on vortex dynamics.}

\duowen{In a different approach within particle-based fluid dynamics, \citet{de2015power} introduced the concept of power particles. These particles are utilized to partition the computational domain into power diagrams, which ensure an even distribution of particles and enable precise pressure solving. Subsequent enhancements have been made, including the acceleration of power diagram computations on GPUs \cite{zhai2018fluid}, and the refinement of free-surface treatment through sphere clamping \cite{levy2022partial}, as opposed to the use of ghost particles. Our method takes advantage of this approach but capable of preserving energy and vorticity through the adaption of a flow map advection and a gauge variable in fluid simulation}

\paragraph{Gauge-based fluid simulation}
Flow maps are particularly relevant when considering the concept of the \textit{impulse variable}. This term was first introduced in \cite{buttke1992lagrangian} and offers an alternative formulation of the incompressible Navier-Stokes Equation through the use of a gauge variable and gauge transformation \cite{oseledets1989new, roberts1972hamiltonian, buttke1993velicity}. Various aspects of gauge freedom have been explored, including its application to surface turbulence \cite{buttke1993velicity, buttke1993turbulence}, numerical stability \cite{weinan2003gauge}, and fluid-structure interactions \cite{cortez1996impulse, summers2000representation}. More recent research by \citet{saye2016interfacial, saye2017implicit} has utilized gauge freedom to address interfacial discontinuities in density and viscosity in free surface flows and fluid-structure coupling.

The concept of \textit{gauge freedom} was revisited in the field of computer graphics by \citet{feng2022impulse}, \citet{yang2021clebsch}, and \citet{nabizadeh2022covector}. However, these methods encountered limitations due to the constraints of the advection schemes employed. NFM \cite{deng2023fluid} addresses this issue by introducing a state-of-the-art neural hybrid advection scheme using flow maps. Despite its advancements, NFM is constrained by the requirements for neural buffer storage and extended training times.

In contrast, our method adopts a more intuitive approach by representing flow maps using Lagrangian particles. This significantly reduces the computational costs associated with NFM, while maintaining its high-quality results.

\paragraph{Flow-map method}
{The concept of a flow map, initially known as the method of characteristic mapping (MCM), was first introduced by \citet{wiggert1976numerical}. This method diminishes numerical dissipation by employing a long-range mapping to track fluid quantities, thereby reducing the frequency of interpolations required. This idea was later adapted for the graphics community by \citet{tessendorf2011characteristic}. Subsequent research \cite{hachisuka2005combined, sato2017long, sato2018spatially, tessendorf2015advection} in this area utilized virtual particles to track the flow map, yet faced substantial computational demands in terms of memory and time.}

{A bidirectional flow map approach was developed by \citet{qu2019efficient}, drawing inspiration from BFECC \cite{kim2006advections}, to enhance the mapping's accuracy. Building on this, \citet{nabizadeh2022covector} combined the impulse fluid model \cite{cortez1996impulse} with the flow map concept. In NFM \cite{deng2023fluid}, the authors introduced the concept of a \textit{perfect flow map} and employed a neural network to efficiently compress the storage of velocity fields required for reconstructing the flow map with high precision. These methods extensively use virtual particles to trace the flow map and employ various techniques to minimize the costs and errors associated with this approach.}

{Our research diverges from these methods by directly tracking the flow map on particles. This approach proves to be more intuitive for flow map tracking and significantly reduces computational costs without compromising accuracy.}
